Predictive Energy Management for Battery Electric Vehicles with Hybrid Models

This paper addresses the problem of predicting the energy consumption for the drivers of Battery electric vehicles (BEVs). Several external factors (e.g., weather) are shown to have huge impacts on the energy consumption of a vehicle besides the vehicle or powertrain dynamics. Thus, it is challenging to take all of those influencing variables into consideration. The proposed approach is based on a hybrid model which improves the prediction accuracy of energy consumption of BEVs. The novelty of this approach is to combine a physics-based simulation model, which captures the basic vehicle and powertrain dynamics, with a data-driven model. The latter accounts for other external influencing factors neglected by the physical simulation model, using machine learning techniques, such as generalized additive mixed models, random forests and boosting. The hybrid modeling method is evaluated with a real data set from TUM and the hybrid models were shown that decrease the average prediction error from 40% of the pure physics model to 10%.

==> abbrv.tex <==
\phantomsection \addcontentsline{toc}{chapter}{List of Abbreviations}
\renewcommand\refname{Abkürzungsverzeichnis} \chapter*{List of Abbreviations}
\begin{acronym}[.................]
		\setlength{\itemsep}{-\parsep}
		\acro{AIC}{Akaike Information Criterion}
		\acro{APE}{Absolute Percentage Error}
		\acro{ARIMAX}{Autoregressive Integrated Moving Average with Explanatory Variable}		
		\acro{BEVs}{Battery Electric Vehicles}
		\acro{BIC}{Bayesian Information Criterion}
		\acro{CAFE}{Corporate Average Fuel Economy}
		\acro{DNN}{Deep Neural Network}
		\acro{EDF}{Effective Degree of Freedom}
		\acro{FASTSim}{Future Automotive Systems Technology Simulator}
		\acro{GAMMs}{Generalized Additive Mixed Models}
		\acro{GEE}{Generalized Estimating Equation}
		\acro{GHG}{Greenhouse Gas}
		\acro{GLMM}{Generalized Linear Mixed Model}
		\acro{GPS}{Global Positioning System}
		\acro{HEVs}{Hybrid Electric Vehicle}
		\acro{ICC}{Intra-class Correlation Coefficient}
		\acro{LMM}{Linear Mixed Model}
		\acro{LOOCV}{Leave-one-out Cross-validation}
		\acro{LSTM}{Long Short-Term Memory}
		\acro{MLR}{Multiple Linear Regression}
		\acro{ML}{Maximum Likelihood}
		\acro{NN}{Neural Network}
		\acro{OLS}{Ordinary Least Squares Regression}
		\acro{PHEVs}{Plug-in Hybrid Electric Vehicles}
		\acro{Q-Q Plot}{Quantile-Quantile Plot}
		\acro{REML}{Restricted Maximum Likelihood}
		\acro{RF}{Random Forests}
		\acro{RMSE}{Root Mean Squared Error}
		\acro{SOC}{State of Charge}
		\acro{SVM}{Support Vector Machine}
		\acro{VED}{Vehicle Energy Dataset}
		\acro{VMT}{Vehicle Miles Traveled}
		\acro{XGBoost}{eXtreme Gradient Boosting}
\end{acronym}

==> methodology.tex <==
\chapter{Methodology}\label{methodology}
This chapter describes the methodology that	has	been used for the proposed hybrid modeling approach. More specifically, Section \ref{Exploratory data analysis} describes the data exploratory process, Section \ref{Data preprocessing} describes how the data is being pre-processed, Section \ref{Previous attempt} lists the previously used but not utilized anymore approaches, Section \ref{Hybrid modeling for energy consumption estimation} presents in detail how the hybrid modeling works and finally in Section \ref{Evaluation}, the way to evaluate the models is shown.

\section{Exploratory data analysis}\label{Exploratory data analysis}
Data exploration allows for a deeper understanding of a dataset, making it easier to navigate and use the data later. Before modeling the data, it also gives insight into all of the data and the numerous interactions between the data elements.

\subsection{TUM dataset}

Figure \ref{fig:single_tum} shows the data for a single trip in TUM dataset. Each column is a time series, which means the observations are measured repetitively over time. As the total power or total energy consumed is not available in the TUM dataset, the energy consumption is calculated based on the formulas:

\begin{equation}
P(t) = I(t)V(t)
\label{eq:phy_1}
\end{equation}

where \(P(t)\) is the power at time \(t\) measured in watt(W), \(I(t)\) is the battery current at time \(t\) measured in amp(A), \(V(t)\) is the battery voltage at time \(t\) measured in volt(V).\\

\begin{equation}
E(t) = P(t)t
\label{eq:phy_2}
\end{equation}

where \(E(t)\) is the energy consumption at time \(t\), \(P(t)\) is the power at time \(t\) measured in watt(W), and \(t\) is time interval.\\

\begin{figure}[!htb]
\centering
\includegraphics[width=15cm]{figures/single.png}
\caption{Example single trip in TUM dataset.}
\label{fig:single_tum}
\end{figure}

The difference between the real energy consumption and physics-based simulation model estimations is the response, it is calculated by subtracting the physics-based simulation model predictions from the real energy consumption:

\begin{equation}
Residual_{Phy}(t) = RealEnergy(t) - Phy_{pred}(t)
\label{eq:residual}
\end{equation}

where \(t\) is time.\\

The elevation of a vehicle is not of primary interest, but the changes of the elevation. The column \(DiffElevation\) is therefore added to the data frame, and is calculated by subtracting the elevation values at each time point by the previous time point's value:

\begin{equation}
DiffElevation(t) = Elevation(t) - Elevation(t-1)
\label{eq:DiffElevation}
\end{equation}

where \(t\) is time.\\

To understand more how the variables are distributed and the correlations between them, data exploratory is carried out. The column \(Physical.predicted\) is the forecasts from the physics-based model and is inserted to the data frame. Figure \ref{fig:data_type_tum} shows the data type of all the columns available in TUM dataset, Figure \ref{fig:distri_tum} shows the marginal distributions of the numeric variables in TUM dataset, and the correlations between them is shown in Figure \ref{fig:corr_tum}. \\

\begin{figure}[!htb]
\centering
\includegraphics[width=15cm]{figures/Data_type.PNG}
\rule{0in}{1.2em}$^\dag$\scriptsize The original TUM dataset was measured once per 0.1 seconds, the figure shows the one already reduced to once per second. The energy will therefore equal to the power used, which doesn't need to multiply the time. \\ 
\caption{Data type of the columns in TUM dataset.}
\label{fig:data_type_tum}
\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=15cm, height=11cm]{figures/distr.png}
\caption{Marginal distribution of numeric variables for TUM dataset.}
 \label{fig:distri_tum}
\end{figure}


\begin{figure}[!htb]
\centering
\includegraphics[width=15cm, height=16cm]{figures/corr.png}
\caption{Correlation matrix of numeric variables for TUM dataset.}
 \label{fig:corr_tum}
\end{figure}


To see how many trips are recorded in summer or winter, in different weather, and in different driving areas, the histograms of these variables are shown in Figure \ref{fig:num_seasonality}, \ref{fig:num_weather}, and \ref{fig:num_route}.\\

\begin{figure}[!htb]
\centering
\includegraphics[width=12cm]{figures/num_seasonality.png}
\caption{Percentages of the trips per seasonality in TUM dataset.}
 \label{fig:num_seasonality}
\end{figure}



\begin{figure}[!htb]
\centering
\includegraphics[width=12cm]{figures/num_weather.png}
\caption{Percentages of the trips per weather in TUM dataset.}
 \label{fig:num_weather}
\end{figure}


\begin{figure}[!htb]
\centering
\includegraphics[width=12cm]{figures/num_route.png}
\caption{Percentages of the trips per route in TUM dataset.}
 \label{fig:num_route}
\end{figure}


Furthermore, the heating power and air conditioner power are the two main resources where energy from the battery consumed the most besides propulsion of the vehicle and are not considered by the physics-based simulation model. It is therefore important to know if two signals are usable for explanation purposes from the dataset. Ambient temperature and time are plotted against the air conditioner power and heating power respectively to check the validity of the signals. Figure \ref{fig:comp_new_tum} shows the scatter plot and different smoothers between the variables mentioned above and Figure \ref{fig:sum_tum} shows the summary statistics of heating power and air conditioner power for each ambient temperature. For Figure \ref{fig:comp_new_tum} (c), ambient temperature v.s. heating power, around ambient temperature 20 degrees, the heating power consumed is even larger than the one in the lower temperature, it's not realistic. After further deep-diving into the dataset for each trip separately, the signals may not be accurate. The assumption is also confirmed by the authors who published the dataset. The main reason is that the high voltage heater is not installed on the vehicle as standard in BMW i3, so the communication is translated via a gateway, which results in erroneous signals in some trips. The heating power and air conditioner power signals are therefore no longer used in this study.   

\begin{figure}[!htb]
\centering
\subfloat[(a) Aircon v.s. Temperature]{\includegraphics[height=6cm]{figures/smooth_t_aircon.png}}
\subfloat[(b) Aircon v.s. Time]{\includegraphics[height=6cm]{figures/smooth_time_aircon.png}}

\subfloat[(c) Heating v.s. Temperature]{\includegraphics[height=6cm]{figures/smooth_t_heat.png}}
\subfloat[(d) Heating v.s. Time]{\includegraphics[height=6cm]{figures/smooth_time_heat.png}}
\caption{Scatter plot and different smoothers between variables in TUM dataset.}
\label{fig:comp_new_tum}
\end{figure}



\begin{figure}[!htb]
\centering
\subfloat[(a) Heating v.s. Temperature]{\includegraphics[height=6cm]{figures/tum_sum_amb_heat.png}}
\subfloat[(b) Aircon v.s. Temperature]{\includegraphics[height=6cm]{figures/tum_sum_amb_aircon.png}}
\caption{Summary statistics of heating power and air conditioner power for each ambient temperature for TUM dataset.}
\label{fig:sum_tum}
\end{figure}


\subsection{VED dataset}
The same data exploratory procedure is also conducted on the VED dataset. Figure \ref{fig:single_us} shows an example of a single trip in VED dataset. Each column is measured repetitively over time.\\


\begin{figure}[!htb]
\centering
\includegraphics[width=15cm]{figures/single_2.png}
\caption{Example single trip in VED dataset.}
 \label{fig:single_us}
\end{figure}

The columns \(Residual\) and \(DiffAltitude\) are added to the data by using Formula \ref{eq:residual} and Formula \ref{eq:DiffElevation} and the column \(Physical.predicted\) is the forecasts from the physics-based simulation model. Figure \ref{fig:data_type_us} shows the data type of the variables in the VED dataset, Figure \ref{fig:distri_us} shows the marginal distributions of the numeric variables in VED dataset, and the correlations between them is shown in Figure \ref{fig:corr_us}. \\

\begin{figure}[!htb]
\centering
\includegraphics[width=15cm]{figures/data_type_2.PNG}
\caption{Data type of the columns in VED dataset.}
 \label{fig:data_type_us}
\end{figure}


\begin{figure}[!htb]
\centering
\includegraphics[width=15cm, height = 13cm]{figures/distri_2.png}
\caption{Marginal distribution of numeric variables for VED dataset.}
 \label{fig:distri_us}
\end{figure}


\begin{figure}[!htb]
\centering
\includegraphics[width=15cm]{figures/corr_2.png}
\caption{Correlation Matrix of numeric variables for VED dataset.}
 \label{fig:corr_us}
\end{figure}

The heating power and air conditioner power are again checked against time and ambient temperature to ensure the plausibility of the two signals. Figure \ref{fig:comp_new_us} shows the scatter plots and different smoothers between the variables mentioned above in VED dataset and Figure \ref{fig:sum_ved} shows the summary statistics of heating power and air conditioner power for each ambient temperature. For the Figure \ref{fig:comp_new_us} (d), it is interesting that after around 3000 seconds, there is no heating power used anymore. To further investigate this, the heating power against time and mean ambient temperature is plotted out and is shown in Figure \ref{fig:heat_tem_time}. The situation is plausible as the longer trips are driving in the warmer temperature which don't require heater. There are no more obvious abnormal patterns being spotted. However, those two signals are still treated with caution when it comes to interpretation.

\begin{figure}[!htb]
\centering
\subfloat[(a) Aircon v.s. Temperature]{\includegraphics[height=6cm]{figures/smooth_t_aircon2.png}}
\subfloat[(b) Aircon v.s. Time]{\includegraphics[height=6cm]{figures/smooth_time_aircon2.png}}

\subfloat[(c) Heating v.s. Temperature]{\includegraphics[height=6cm]{figures/smooth_t_heat2.png}}
\subfloat[(d) Heating v.s. Time]{\includegraphics[height=6cm]{figures/smooth_time_heat2.png}}
\caption{Scatter plot and different smoothers between variables in VED dataset.}
\label{fig:comp_new_us}
\end{figure}


\begin{figure}[!htb]
\centering
\subfloat[(a) Heating v.s. Temperature]{\includegraphics[height=6cm]{figures/ved_sum_amb_heat.png}}
\subfloat[(b) Aircon v.s. Temperature]{\includegraphics[height=6cm]{figures/ved_sum_amb_aircon.png}}
\caption{Summary statistics of heating power and air conditioner power for each ambient temperature for VED dataset.}
\label{fig:sum_ved}
\end{figure}

\begin{figure}[!htb]
\centering
\includegraphics[width=12cm,height=8cm]{figures/heat_tem_time.png}
\caption{Heating power against time and mean ambient temperature.}
 \label{fig:heat_tem_time}
\end{figure}


\section{Data preprocessing}\label{Data preprocessing}
As the dataset may contain redundancy such as irregular data, missing values, or outliers that may cause the model to overfit or underfit during training, the data pre-processing is conducted before data modeling. 

\subsection{Data downsampling}
The original TUM dataset was measured once per 0.1 seconds and the original VED dataset was measured once per second. For efficiency purposes, the two original datasets are reduced to once per 10 seconds. The reducing method is done by sampling a record of every 100 records for the TUM dataset and 10 records for the VED dataset. Furthermore, another reason to do this is that it would be more realistic as in real life the data won't be that accurate.

\subsection{Data elimination}
After doing further research, some unrealistic values were detected in the TUM dataset. The erroneous signals will significantly influence the results of the analysis, so trip by trip examination was performed to ensure the quality of the datasets. (e.g., 2014 BMW i3 is equipped with the heater that can deliver a maximum of 7 kW, any values exceeding this value are considered as recording error).
\\\\
Furthermore, the trips which contain battery charging pattern (the vehicle is standing still (i.e., velocity is 0) and the energy is very negative) are discarded as the timing when will the driver start charging is hard to predict and the datasets only have a few trips with battery charging pattern. Figure \ref{fig:charging} is an example of when battery charging occurs during a trip. When the time is after around 2800 seconds, the velocity is 0, and the energy is very negative, this is an indication that the vehicle is charging during the time period.

\begin{figure}[!htb]
\centering
\includegraphics[width=16cm,height=12cm]{figures/charging.png}
\caption{Example of battery charging pattern occurs during a trip.}
 \label{fig:charging}
\end{figure}


\subsection{Missing value imputation}
The VED dataset contains missing values, which result in an incomplete dataset. Instead of carrying the last observation forward which can introduce bias in analysis and perform poorly when data has a visible trend, linear interpolation is utilized for missing value imputation taking adjacent values. Data with the trend and without seasonality are mostly imputed by linear interpolation, and the formula for linear interpolation is:

\begin{equation*}
{\displaystyle y=y_{0}+(x-x_{0}){\frac {y_{1}-y_{0}}{x_{1}-x_{0}}}={\frac {y_{0}(x_{1}-x)+y_{1}(x-x_{0})}{x_{1}-x_{0}}}}
\end{equation*}

where \(x\) is the known value, \(y\) is the unknown value, \(x_0\) and \(y_0\) are the coordinates that are below the known \(x\) value, and \(x_1\) and \(y_1\) are the coordinates that are above the \(x\) value \cite{noor2015comparison}.



\subsection{Categorical features encoding}
The columns weather, route, and seasonality are in qualitative form and do not have any ranking for category values, these columns are converted into numerical data using one-hot encoding. With one-hot encoding, each categorical value is converted into a new categorical column and assigned a binary value of 1 or 0 to those columns. Each integer value is represented as a binary vector. All the values are zero, and the index is marked with a 1.



\subsection{Feature scaling}
Feature scaling is a method used to normalize the range of independent variables or features of data. Generally speaking, the models which calculate some kind of distance as part of the algorithm needs the data to be scaled, such as \ac{SVM}, Ridge, or Lasso regressions. Tree-based models (e.g., random forest, boosting) where each node is split based on the condition don’t need the features to be scaled because the model accuracy doesn't depend on the range. In regression, on the other hand, scaling would be not necessary when the scale is meaningful. In this thesis, scaling of the features is not performed as the effects of each feature are of interest. 


\section{Previous attempt}\label{Previous attempt}
The section lists the previously used but not utilized anymore approaches. The reasons why they are abandoned are described in more detail in the corresponding subsection.

\subsection{Short-term time series prediction}
Short-term time series prediction is a method to fit a model on each cluster or each subject. That is to say, in the study, each trip has its own time series models. The commonly used time series model including \ac{ARIMAX}, \ac{LSTM}, \ac{XGBoost}, random forest were applied previously. These models fit very well on each of the trips but failed to generalize to the other trip, which shows a very high error rate for testing trips. If one wants to predict the energy consumption for a specific trip only for the next few time points, the method can be used. However, it is not well-suitable if a person wants to know if he or she can reach the final destination as planned in the beginning of a trip.

\subsection{Trip IDs as feature}
The approach is not applicable if one wants to predict the trip, not in the training dataset. In this thesis, the trips are divided into training and testing datasets to evaluate the prediction accuracy and Trip ID is unique for each trip, the approach is therefore not applicable.


\subsection{Air conditioner power and heating power modeling}
The modeling approach was used previously, but with the assumption that the heating power and air conditioner power signals are reliable. Those two signals are positive-definite and therefore GAMM with hurdle model is used. The hurdle model allows observed zeros to
arise both from the binary part of the model and as an observation from another distribution, e.g., Gamma. This is similar to the situation and data generating process: if the driver will turn on the heater or air conditioner or not, and if he or she turns them on, by how much. The method is no longer considered as the heating power and air conditioner power signals contain measurement errors. 


\section{Hybrid modeling for energy consumption estimation}\label{Hybrid modeling for energy consumption estimation}
The energy consumption of a BEV depends upon a number of factors like road elevation, vehicle speed, vehicle acceleration, etc. These factors have a non-linear relation among them as they vary a lot in the real world. Therefore, to accurately estimate their non-linear relation, a low-fidelity physics-based simulation model is utilized to capture the basic vehicle and powertrain dynamic. However, the physics-based simulation model can show a large difference to the real energy consumption as the physics-based simulation model is not fine-grained according to a specific vehicle. Furthermore, the energy consumed also depends on external factors, like weather, ambient temperature, etc., which are not considered by the physics-based simulation model. Those possible deviations from reality and external influential factors are incorporated into the prediction of energy consumption by utilizing machine learning corrective models. 


\subsection{Low-fidelity physics-based model simulation}
The physics-based simulation model is implemented in MATLAB containing a Battery Electric Vehicle (BEV) model and its components such as motor, high voltage battery, and longitudinal vehicle. The model is expected to capture the basic vehicle and powertrain dynamics. The drawback of the physics-based simulation model is that it doesn't have an air conditioner and heating power components and external factors like ambient temperature (e.g., with the potential to influence battery efficiency) are not taken into consideration. The physics-based simulation model will therefore show a large deviation from the real energy consumed during a trip.
\\\\
The physics-based simulation model takes the following variables as inputs from the dataset: velocity, elevation, and time. The parameters related to the vehicle like the vehicle's weight are roughly calibrated according to the 2014 BMW i3 as the TUM dataset is using this vehicle as to the testing vehicle (some parameters are unknown for the 2014 BMW i3, like efficiency maps of the electric motor, can only be calculated approximately). The vehicles used for the trips in the VED dataset are unknown, and therefore 2014 BMW i3 is still assumed. Some of the parameters set for the physics-based simulation model are shown in Table \ref{tab:bmw_i3}. The physics-based simulation model will output the parameters related to the battery, such as SOC, battery voltage, battery current, and battery temperature based on the theories in Physics (e.g., Hamiltonian and Pontryagin's minimum principle \cite{zhang2020computationally}). From the output information of the physics-based simulation model, the estimated energy consumption from the physics-based simulation model can be calculated for each timestamp by using the Formula \ref{eq:phy_1} and Formula \ref{eq:phy_2}. \\

Besides the parameters related to the vehicle itself, regenerative braking (recuperation) can also have a huge impact on the energy consumption of BEVs and is assumed 50\% for the TUM dataset as the dataset contains more trips with higher ambient temperature, and is set to 0\% for VED dataset as the dataset contains more trips driving in low temperature (the value represents the percentage of the energy the battery can get back from braking). Regenerative braking is the recovery of kinetic energy during braking. The steeper the downhill is, the more energy the battery can get back from the braking behavior. Furthermore, low battery temperature can influence the capability to recuperate in order to protect the battery from accelerated aging, which ultimately leads to less energy regeneration back to the battery \cite{steinstraeter2021effect}.
\\

Figure \ref{fig:example_outputs} shows the example outputs from the physics-based simulation model for a single trip. SOC is the battery's state of charge, which is the level of charge of an electric battery relative to its capacity; dSOC is the changes of SOC; I is the battery' current; Voc is the open-circuit voltage, the maximum voltage available from a solar cell; V is the battery's voltage, respectively.

\begin{figure}[!htb]
\centering
\includegraphics[width=15cm]{figures/example_output.jpg}
\caption{Example outputs from the physics-based simulation model for a single trip.}
 \label{fig:example_outputs}
\end{figure}



\begin{table}[!htb]
\centering
\caption{\label{tab:bmw_i3}Vehicle specifications.}
\vspace*{5mm}
\begin{tabular}{@{} l L L L @{} >{\kern\tabcolsep}l @{}}    \toprule
\emph{Property} & \emph{Value}   \\\midrule
Vehicle mass in kg    & 1345      \\ 
Wheel diameter in m  & 0.6996  \\ 
Drag coefficient  & 0.22  \\ 
Number of wheels   & 4  \\ 
Rotational mass ratio  & 5  \\ 
Battery cell capacity in Ah  & 120  \\ 
Battery mass in kg & 450  \\ 
Number of cells in battery in parallel & 1 \\ 
 Number of cells in battery in series & 96 \\\bottomrule
 %\hline
\end{tabular}
\end{table}


\subsection{Machine learning corrective model}
TUM dataset and VED dataset contain different amounts of information (columns), and the driving vehicles are unknown for the VED dataset, it is, therefore, hard to combine these two datasets to form a single statistical corrective model. However, in order to fully evaluate the proposed methods, the two datasets are analyzed separately.
\\\\
Heating power and air conditioner power are the two main resources of energy consumption besides propulsion (driving needed energy), and the weather and ambient temperature are the main factors that influence if the driver will turn on the heater or air conditioner or not. The difference between the real energy consumption and the physics-based simulation model forecasts can therefore be partially estimated by those external factors (e.g., weather, ambient temperature). Furthermore, to further improve the prediction accuracy of the energy consumption of BEVs, the physics-based simulation model's inputs: time, elevation, and speed are also taken as inputs to the machine learning corrective models to account for possible deviations due to the reason that the physics-based simulation model is not fine-grained.
\\\\
The information available at the beginning of the trip are the only inputs allowed to use. Weather and ambient temperature information can be gotten from the weather forecast, the rough speed (maximum speed allowed for a segment of a road for example), and elevation can also be gotten from some online location platforms, like Here.com.


\subsubsection{Heterogeneity test}
The differing habits of different drivers can lead to variations in the difference between the real energy consumption and physics-based simulation model predictions (i.e., \(Residual_{Phy}\)). If the driver is sensitive to the ambient temperature, for example, the heater will be turned on very often with high energy consumed during winter, and the same holds for the air conditioner during summer. The difference between the real energy consumption and physics-based model predictions will therefore be larger. As the data is labeled as trip specific, so the trip IDs is used to represent different driving behavior and characteristics. Also, the heterogeneity can potentially be induced by another factor "driving area", it's also tested for heterogeneity. Those differences between the trips may be represented by a stochastic parameter with a normal distribution if no other disturbance exists. To test the heterogeneity between the trips, the intra-class correlation coefficient (ICC) is utilized.
\\\\
ICC is usually calculated for the null model, the simple baseline linear mixed models with no covariates and only random intercept are therefore used:
\begin{equation*}
\begin{aligned}
y_{ij} = \gamma_{00} + \mu_{0i} + \epsilon_{ij}
\end{aligned}
\end{equation*}

where \(y_{ij}\) is the \(j\)th observation of \(Residual_{Phy}\) among the trips in the \(i\)th group (e.g., corresponding to a particular trip ID, driving area); \(\gamma_{00}\), known as the fixed portion, is the overall
mean of \(Residual_{Phy}\); \(\mu_{0i}\) is a family effect shared by all members of
group \(i\), which is assumed to vary following a normal distribution
with a mean of zero and a variance of \(\sigma_b^2\); and \(\epsilon_{ij}\) is the individual disturbance term, which is distributed independently and normally
with a mean of zero and a variance of \(\sigma_\omega^2\).\\

The heterogeneity induced by trip IDs and different driving areas effects will be exhibited only in
the random intercept components of this model; this is a simple approach, but it is helpful for understanding the distribution of the variability in energy efficiency.\\


Among the 65 studied BEVs in the TUM dataset, the ICC values for the machine learning corrective model corresponding to the driving area and trip IDs are summarized in Table \ref{tab:h_tum}. The ICC value for the driving area is
2.6\%, which means that different driving district explains roughly 2.6\% of the variation. The ICC value for the trip ID is 7.1\%, which means that 7.1\% of the variation in the \(Residual_{Phy}\) deviations per trip was due to the drivers’ personal characteristics.\\


\begin{table}[!htb]
\centering
\caption{\label{tab:h_tum}ICCs for \(Residual_{Phy}\) estimation for TUM dataset.}
\vspace*{5mm}
\begin{tabular}{@{} l L L L @{} >{\kern\tabcolsep}l @{}}    \toprule
\emph{Cluster} & \emph{ICC(\%)}   \\\midrule
 Driving area    & 2.6      \\ 
 Trip IDs & 7.1 \\\bottomrule
 %\hline
\end{tabular}
\end{table}


The same heterogeneity test is also applied to the VED dataset. Among the 460 studied BEVs in the VED dataset, the ICC value for the machine learning corrective model corresponding to the trip IDs is shown in Table \ref{tab:h_ved}.\\


\begin{table}[!htb]
\centering
\caption{\label{tab:h_ved}ICCs for \(Residual_{Phy}\) estimation for VED dataset.}
\vspace*{5mm}
\begin{tabular}{@{} l L L L @{} >{\kern\tabcolsep}l @{}}    \toprule
\emph{Cluster} & \emph{ICC(\%)}   \\\midrule
 Trip IDs & 8 \\\bottomrule
 %\hline
\end{tabular}
\end{table}

The ICC value for the trip IDs is 8\% for the VED dataset, which means that 8\% of the variation in the response deviations per trip was due to the drivers’ personal preferences. 
\\\\
ICC values range from zero to one (i.e., 0 to 100 \%). There are different viewpoints on the definition of the low or high value of ICC. For example, a common rule of thumb for a low ICC is 5 \%, \cite{cohen2013statistical} recommended that the ICC should be considered significant if larger than 5.9\%, and various other authors suggest that multilevel models are not appropriate when intra-class correlation (ICC) is low (or 0). \cite{nezlek2008introduction} argues that it is a risky assumption to base a decision not to employ multilevel modeling on a low or zero ICC. The fact that there is little or no between-group
variance in a measure does not mean that the relationship between this
measure and another measure is the same across all groups. By extension, even if there is no between-group variance for any of the variables of interest, connections between and among them cannot be assumed to remain constant across groups. Therefore the multilevel structure is still considered instead of treating the observations as independent.
\\\\
Many statistical models have been proposed to handle correlated data, such as the most well-known mixed-effects models. Instead of using only one type of model to construct the machine learning corrective model, it is also worth trying the other models and comparing which model is more efficient and performs the best.  


\subsubsection{Generalized additive mixed models (GAMMs)}
\paragraph{Model formulation}$ $\newline
The histogram of the response (i.e., \(Residual_{Phy}\)) for both datasets is continuous and is not skewed, the general Gaussian family is applied. The model formulation for the generalized additive mixed-effects model with Gaussian family fitted on TUM dataset is shown in Formula \ref{eq:formulation_mixed}. In addition, Student’s t family will be used instead if the Gaussian family doesn't fit the data well. Furthermore, it is believed that the effect of elevation of a vehicle on the energy consumption also depends on battery temperature, the interaction term of \(AmbientTemperature\) (with the potential to influence the battery temperature) and \(DiffElevation\) is added to the models.


\begin{equation}
\begin{split}
Residual_{Phy}TUM_{ij} = \beta_{0} + f_1(Time_{ij}) + f_2(AmbientTemperature_{ij}) + f_3(Velocity_{ij}) + \\f_4(DiffElevation_{ij}) + f_5(Time_{ij}) \cdot SeasonalityWinter_i +\\ f_6(AmbientTemperature_{ij}) \cdot SeasonalityWinter_i \\+ f_7(AmbientTemperature_{ij} \cdot DiffElevation_{ij}) + WeatherCloudy_i +\\ WeatherDark_i + WeatherDarkRainy_i + WeatherRainy_i + WeatherSlightCloudy_i + \\WeatherSunny_i + WeatherSunrise_i + WeatherSunset_i + b_{0i}+ \epsilon_{ij}
\end{split}
\label{eq:formulation_mixed}
\end{equation}


where \(f_1,f_2,f_3,f_4,f_5,f_6,f_7\) are smooth functions estimated by restricted maximum likelihood, and \(b_{0i} \sim \mathcal{N}(0,\sigma_b^2)\), \(\epsilon_{ij} \sim \mathcal{N}(0,\sigma^2)\).\\


As the VED dataset contains less information compared to the TUM dataset, the formulation of the model is different from the TUM dataset. The model formulation for the generalized additive mixed-effects model with Gaussian family fitted on VED dataset is shown in Formula \ref{eq:formulation_mixed_VED}.

\begin{equation}
\begin{split}
Residual_{Phy}VED_{ij} = \beta_{0} + f_1(Time_{ij}) + f_2(AmbientTemperature_{ij}) + f_3(Speed_{ij}) + \\f_4(DiffAltitude_{ij}) + f_5(AmbientTemperature_{ij} \cdot DiffAltitude_{ij}) + b_{0i} + \epsilon_{ij}
\end{split}
\label{eq:formulation_mixed_VED}
\end{equation}


where \(f_1,f_2,f_3,f_4,f_5\) are smooth functions estimated by restricted maximum likelihood, and \(b_{0i} \sim \mathcal{N}(0,\sigma_b^2)\) and \(\epsilon_{ij} \sim \mathcal{N}(0,\sigma^2)\).



\paragraph{Model selection}$ $\newline
Model selection is the task of selecting a statistical model from a set of candidate models. The GAMMs are fitted using REML and are not comparable if the fixed effects are different. In addition, when comparing models, the models are usually re-fitted using ML. The random effect component is tested for these models using Akaike information criterion (AIC) and Bayesian information criterion (BIC). Table \ref{tab:model_select_tum} and Table \ref{tab:model_select_ved} show the AIC and BIC values for GAMMs fitted using ML with random effect and without random effect on TUM and VED dataset, respectively. \\


\begin{table}[!htb]
\centering
\caption{\label{tab:model_select_tum}AIC and BIC values for GAMMs fitted on TUM dataset.}
\vspace*{5mm}
\begin{tabular}{@{} l L L L @{} >{\kern\tabcolsep}l @{}}    \toprule
& \emph{With random effect} & \emph{ Without random effect }   \\\midrule
 AIC & 196545.6 & 196628.5\\
 BIC & 196997.8 & 196820.3\\\bottomrule
% \hline
\end{tabular}
\end{table}


\begin{table}[!htb]
\centering
\caption{\label{tab:model_select_ved}AIC and BIC values for GAMMs fitted on VED dataset.}
\vspace*{5mm}
\begin{tabular}{@{} l L L L @{} >{\kern\tabcolsep}l @{}}    \toprule
& \emph{With random effect} & \emph{ Without random effect }   \\\midrule
 AIC & 512068.7 & 513390.2\\
 BIC & 515036.7 & 513788.8\\\bottomrule
 %\hline
\end{tabular}
\end{table}

The smaller the AIC or BIC, the better the model is. Although the two criteria are in favor of different models, the AIC is chosen in this case. \cite{shmueli2010explain} gives a good summary in this respect: The AIC is better suited to model selection for prediction as it is asymptotically equivalent to leave-one-out cross-validation in regression, or one-step-cross-validation in time series. On the other hand, it might be argued that the BIC is better suited to model selection for the explanation, as it is consistent. Therefore, the AIC value is chosen as the aim is on the prediction of the real energy consumption of BEVs.

\subsubsection{Random forest}
The same set of variables are used as inputs for the random forest model.

\paragraph{Hyperparameter tuning}$ $\newline
Although the official page of the random forest algorithm: \cite{RandomForests}, states that random forest does not overfit, and one can use as many trees as he wants. \cite{segal2004machine} argues that it overfits some noisy datasets.
To test if the result is sensitive to different settings of the hyperparameters, different values for the hyperparameters are used and run instead of finding an optimal combination of hyperparameters using grid search or random search. Table \ref{table:hyper_rf_tum} and Table \ref{table:hyper_rf_ved} show the results for the random forest model fitted on TUM dataset and VED dataset after trying different hyperparameters using leave-one-out cross-validation. The corresponding hyperparameters are varied while having the other hyperparameters fixed at the default setting. Min error is the minimum error from all the cross-validation iterations; Avg error is the average error of the models from all the iterations; Max error is the maximum error from all of the iterations, respectively.
\\\\
The results show that different hyperparameter values of the random forest model don't have a huge impact on the prediction accuracy of the models for both datasets. The values for the hyperparameters are set as: ntrees = 100 and mtry = 4.


\begin{table}[!htb] \centering
%\ra{1.3}
\caption{Hyperparameter tuning for random forest fitted on TUM dataset.}\label{table:hyper_rf_tum}
\vspace*{5mm}
\begin{small}
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}\toprule
 & \textbf{Min Error} & \textbf{Avg Error} & \textbf{Max Error}  \\ \midrule
\underline{\emph{ntrees}} \\
\textbf{50} & 0.0004468371 & 0.100206  &  0.3829159 \\ 
\textbf{100} & 0.0004662982 &  0.1015932 &   0.3880242\\ 
\textbf{200} & 0.00533142  & 0.1033652  &  0.4174384\\ 
\textbf{500} &  0.0007733794 & 0.1035848 & 0.3979348   \\
\underline{\emph{mtry}} \\
\textbf{2} & 0.001757442 &  0.1156016 &  0.3719294 \\ 
\textbf{4} & 0.001878633 & 0.1012515  &  0.3974828 \\ 
\textbf{6} &  0.002236813 &  0.1078142 &  0.4058039\\ 
\bottomrule
\end{tabular}
\end{small}
\end{table}

\begin{table}[!htb] \centering
%\ra{1.3}
\caption{Hyperparameter tuning for random forest fitted on VED dataset.}\label{table:hyper_rf_ved}
\vspace*{5mm}
\begin{small}
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}\toprule
 & \textbf{Min Error} & \textbf{Avg Error} & \textbf{Max Error}  \\ \midrule
\underline{\emph{ntrees}} \\
\textbf{50} & 0.0002665778 &  0.2520502  &  3.324485 \\ 
\textbf{100} & 9.964579e-05 &  0.2523269 &  3.32069 \\ 
\textbf{200} & 5.399716e-05   & 0.2509487 & 3.25237 \\ 
\textbf{500} &  0.0001609709 & 0.251589 &   3.280645 \\
\underline{\emph{mtry}} \\
\textbf{2} & 0.00115318 & 0.255996 &  3.162559 \\ 
\textbf{4} &  4.934035e-05 &  0.2549191 &  3.153511 \\ 
\textbf{6} & 0.0003578167  &  0.2544045 &  3.030754\\ 
\bottomrule
\end{tabular}
\end{small}
\end{table}


\subsubsection{Boosting}
The same set of variables are used as inputs for the boosting model.

\paragraph{Hyperparameter tuning}$ $\newline
With higher chances for the boosting model to overfit the datasets than the random forest model, the sensitivity testing of different values of the hyperparameters for boosting models is carried out. Table \ref{table:hyper_tb_tum} and Table \ref{table:hyper_tb_ved} show the results for the boosting models fitted on TUM dataset and VED dataset after trying different hyperparameters using leave-one-out cross-validation. The corresponding hyperparameters are varied while having the other hyperparameters fixed at the default setting.\\


\begin{table}[!h] \centering
%\ra{1.3}
\caption{Hyperparameter tuning for boosting fitted on TUM dataset.}\label{table:hyper_tb_tum}
\vspace*{5mm}
\begin{small}
\begin{tabular}{@{}lrrrrrrrrrrrr@{}}\toprule
 & \textbf{Min Error} & \textbf{Avg Error} & \textbf{Max Error}  \\ \midrule
\underline{\emph{ntrees}} \\
\textbf{50} & 0.006349241 &  0.115258 &  0.3091608 \\ 
\textbf{100} &  0.001657622 &  0.1033887 &  0.3063349\\ 
\textbf{200} &  0.001490402 & 0.1020025  & 0.3825784 \\ 
\textbf{500} &  0.002198444 &  0.1057451 &   0.4214008 \\
\underline{\emph{nsplit}} \\
\textbf{2} & 0.004818445 & 0.1018676 &  0.3482809 \\ 
\textbf{4} & 0.002303816 &  0.1012444 &  0.309895 \\ 
\textbf{6} & 0.0004681132 &  0.1013352 & 0.3036479 \\ 
\underline{\emph{lambda}} \\
\textbf{0.01} & 0.001186723 & 0.1607713 & 0.346883   \\ 
\textbf{0.05} &  0.001657622 &  0.1033887 &  0.3063349 \\ 
\textbf{0.1} & 0.0001012573 &  0.1021623 & 0.3842218 \\ 
\bottomrule
\end{tabular}
\end{small}
\end{table}


\begin{table}[!h] \centering
%\ra{1.3}
\caption{Hyperparameter tuning for boosting fitted on VED dataset.}\label{table:hyper_tb_ved}
%\vspace*{5mm}
%\begin{small}
\begin{tabular}{c c}
\hline
 & \textbf{Min Error} & \textbf{Avg Error} & \textbf{Max Error}  \\ \hline
\underline{\emph{ntrees}} \\
\textbf{50} & 0.0001395856 &  0.2480316 & 3.606447  \\ 
\textbf{100} & 0.001919118 &  0.2468049  & 3.493305 \\ 
\textbf{200} & 0.0006228978  &  0.2449773 & 3.415275 \\ 
\textbf{500} &  0.0006447636 & 0.2470826 &  3.328492  \\
\underline{\emph{nsplit}} \\
\textbf{2} &0.0001393296  & 0.2430452& 3.473707  \\ 
\textbf{4} & 0.000108314 & 0.2427367  &  3.571641 \\ 
\textbf{6} & 0.00167263 & 0.2440892  & 3.522517 \\ 
\underline{\emph{lambda}} \\
\textbf{0.01} & 0.0003771833 & 0.2487543 & 3.388223  \\ 
\textbf{0.05} & 0.001919118 &  0.2468049 &  3.493305 \\ 
\textbf{0.1} & 0.0007006245 &  0.2444286 & 3.422067 \\ 
\hline
\end{tabular}
%\end{small}
\end{table}

Different hyperparameter values of boosting show little impact on the prediction accuracy of the boosting models for both datasets, the values for the hyperparameters are therefore set as: ntrees = 100, nsplit = 1 and lambda = 0.05.


\section{Evaluation}\label{Evaluation}
To fully evaluate the performance of the predictive models, the leave-one-out cross-validation method is utilized. The error metrics are calculated on the real energy consumption and the hybrid modeling estimated energy consumption. That is to say, the statistical corrective models' forecasts: \(Residual_{Phy}\) are added back to the physics-based simulation model estimations before calculating the prediction accuracy.
\\\\
As the thing, the drivers are concerned the most is if they can reach the final destination as originally planned, the error rate is only calculated at time point \(T\) of a trip (how much the estimated cumulative energy consumption differs from the real cumulative energy consumption at the final destination).



==> symb.tex <==
\phantomsection \addcontentsline{toc}{chapter}{List of Symbols}
\renewcommand\refname{Symbolverzeichnis} \chapter*{List of Symbols}
The list below shows the most important symbols used in this thesis.

\begin{acronym}[.................]
        \setlength{\itemsep}{-\parsep}
        \acro{Time:}\hfill{$t$}
        \acro{Battery current:}\hfill{$I$}
        \acro{Battery voltage:}\hfill{$V$}
        \acro{Total energy:}\hfill{$E$}
        \acro{Total power:}\hfill{$P$}
        \acro{Degrees of freedom:}\hfill{$\nu$}
        \acro{Standard deviation:}\hfill{$\sigma$}
        \acro{Likelihood function:}\hfill{$\mathcal{L}(\cdot)$}
        \acro{Physics-based model predictions:}\hfill{$Phy_{pred}$}
        \acro{Physics-based model predictions' deviations from real value:}\hfill{$Residual_{Phy}$}
\end{acronym}

==> theory.tex <==
\chapter{Theory}\label{theory}
In this chapter will be formally introduced the theories behind the models as well as mathematics estimation and model selection process.

\section{Data structure}
Longitudinal data (or panel data) is data that is collected through a series of repeated observations of the same subjects over some extended time frame \cite{frees2004longitudinal}. The data has the form:

\begin{equation*}
X_{ij}, \quad i = 1,...,n, \quad j = 1,...,n_i
\end{equation*}
where \(i\) is the individual dimension and \(j\) is the time dimension.\\

Longitudinal data varies from cross-sectional data, since it tracks the same subjects over a period of time, whereas cross-sectional data samples different subjects (whether people, businesses, countries or regions) at every point of time.

\section{Modeling alternatives}
\label{modelling alternatives}
In longitudinal studies, the repeated measures for the same person are likely to be more similar due to the fact that the same person is being measured multiple times on the same measurement scale \cite{littell1998statistical}. There are various ways to deal with longitudinal data or correlated data. One simple approach is to aggregate. With this strategy, the model can learn throughout the population, but it won't learn anything unique about specific clusters. For example, suppose 10 students are sampled from each school. Rather than using the individual students’ data, which is not independent, one could take the average of all students within a school. This aggregated data would then be independent. Although aggregate data analysis produces consistent and effective estimates and standard errors, it does not fully utilize all of the data because it merely averages them together.
\\\\
Another approach to longitudinal data is to make a separate model per cluster or subject. For example, one could run six separate linear regressions, one for each school in the sample. Although this works, there are many models, and each of which does not take advantage of the information in data from other clusters, and hence is unable to learn across the population. This can also make the results “noisy” in that the estimates from each model are only based on its own cluster data. 
\\\\
The third approach is to make one global model but put in cluster id as a feature. This is one technique, however it has problems scaling as the cluster size grows, and it can't handle individuals or clusters that aren't in the training dataset \cite{DeySourav}.
\\\\
In order to fully account for the correlations between observations, there are several longitudinal data models have been proposed. The most commonly used approach is mixed models (i.e., multilevel models). Mixed models are a set of models for analyzing observations that are organized into groups. Fixed effects, which are common to any collection of observations, and random effects, which are unique to a single group of observations, characterize these models. These random effects are coefficients drawn from a random distribution, generally a normal distribution. Parameter estimation in these models involves fitting coefficients for the fixed terms and for the variance component describing the distribution of the random effects. Mixed models can thus be applied to certain forms of clustered data and can aid in the resolution of correlated observation issues \cite{bell2019fixed}. 
\\\\
Despite the popularity of mixed models, there are many other models being proposed to deal with longitudinal data. Some of the models are also used and fitted on the datasets, the detailed explanations are provided in the corresponding section below. 


\section{Generalized additive mixed models (GAMMs)}
Among the mixed models, the linear mixed model is the simplest one for modeling longitudinal data and is an extension of simple linear models to allow both fixed and random effects. To model non-Gaussian distributed error terms, generalized linear mixed models (GLMMs) can be used. Generalized Additive Mixed Models (GAMMs), on the other hand, further extends \ac{GLMM} by allowing continuous predictors to have a nonparametric functional impact on the mean response.\\

One advantage of mixed models is that they allow correlated observations within a group or a subject. The intra-class correlation was commonly used to describe how strongly units in the same group resemble each other. If the correlation is zero, that means the observations within-subjects (clusters) are no more similar than observations from different subjects (clusters). The \ac{ICC}, as introduced by \cite{shrout1979intraclass}, is defined as:


\begin{equation}
ICC = \frac{\sigma_b^2}{\sigma^2_\omega + \sigma_b^2}
\end{equation}

where \(\sigma^2_\omega\) is the within-group variance, \(\sigma_b^2\) is the between-group variance, and \(\sigma^2_\omega + \sigma_b^2\) is the total variance. Usually, the ICC is calculated for the null model (“unconditional model”) and is suggested by \cite{raudenbush2002hierarchical}, so the simple baseline linear mixed models with no covariates and only random intercept is used:

\begin{equation}
\begin{aligned}
y_{ij} = \gamma_{00} + \mu_{0i} + \epsilon_{ij}
\end{aligned}
\end{equation}

where \(u_{0i} \sim \mathcal{N}(0,\sigma_b^2)\) and \(\epsilon_{ij} \sim \mathcal{N}(0,\sigma^2_\omega)\).\\


Another benefit of mixed-effects models is the "shrinkage effect", which allows one to have cluster-specific effects while still borrowing strength from population-average effects. This borrowing is especially noticeable for what would otherwise be more extreme clusters and those with less data. That is to say, the estimate of the effect for each subject computed from a mixed-effect model is “pushed” towards the grand mean effect compared to fitting a separate linear model to each subject’s data. 


\subsection{Model formulation}
Suppose that observations of the \(i\)th of \(n\) units consist of an outcome variable \(y_i\) and \(p\) covariates \(x_i = (1, x_{i1},..., x_{ip})^T\) associated with fixed effects and a \(q \times 1\) vector of covariates \(z_i\) associated with random effects. Given a \(q \times 1\) vector \(b\) of random effects, the observations
\(y_i\) are assumed to be conditionally independent with means \(\mathbb{E}(y_i|b) = \mu_i^b\) and variances var\((y_i|b) = \phi m_i^{-1}\upsilon(\mu_i^b)\), where \(\upsilon(\cdot)\) is a specified variance function, \(m_i\) is a prior weight (e.g., a binomial denominator) and \(\phi\) is a scale parameter, and follow a generalized additive mixed model

\begin{equation}
g(\mu_i^b) = \beta_0 + f_1(x_{i1}) + ... + f_p(x_{ip}) + z_i^Tb
\end{equation}

where \(g(\cdot)\) is a monotonic differentiable link function, \(f_j(\cdot)\) is a centred twice-differentiable smooth function, the random effects \(b\) are assumed to be distributed as \(\mathcal{N}\{0, D(\theta)\}\) and \(\theta\) is a
\(c \times 1\) vector of variance components \cite{lin1999inference}.\\


For example, in a longitudinal data set, \(y_{ij}\) is the \(j\)th measurement on the \(i\) subject of a binary response variable \(y\) for each of \(1 \leq j \leq n_i\), \(1 \leq i \leq m\). Let \(x_{1ij}\) and \(x_{2ij}\) be defined similarly for continuous predictors \(x_1\) and \(x_2\). A GLMM for this model is 

\begin{equation}
y_{ij}|b_i \stackrel{ind}{\sim} \textrm{Bernoulli}(\textrm{logit}^{-1}(b_i + \beta_1x_{1ij} + \beta_2x_{2ij})), \quad b_i \stackrel{ind}{\sim} \mathcal{N}(0, \sigma_b^2)
\end{equation}

where \(b_i\) is a random subject intercept.\\

The GAMM for the same data is
\begin{equation}
y_{ij}|b_i \stackrel{ind}{\sim} \textrm{Bernoulli}(\textrm{logit}^{-1}(b_i + f_1(x_{1ij})+ f_2(x_{2ij})), \quad b_i \stackrel{ind}{\sim} \mathcal{N}(0, \sigma_b^2)
\end{equation}

where \(f1\) and \(f2\) are functions that are assumed to be smooth but otherwise arbitrary.\\

There are numerous ways by which \(f1\) and \(f2\) can be estimated. For example, in gammSlice package in R, \(f_1(x_1)+f_2(x_2)\) is modelled using mixed model-based penalised splines:
\begin{equation}
f_1(x_1) + f_2(x_2) = \beta_0 + \beta_{x1}x_1 + \sum_{k=1}^{K_1} u_{1k}z_{1k}(x_1)+ \beta_{x2}x_2 + \sum_{k=1}^{K_2} u_{2k}z_{2k}(x_2)
\end{equation}

where \(u_{1k} \stackrel{ind}{\sim} \mathcal{N}(0, \sigma_1^2)\), \(1 \leq k \leq K_1\) and \(u_{2k} \stackrel{ind}{\sim} \mathcal{N}(0, \sigma_2^2)\), \(1 \leq k \leq K_2\) \cite{pham2018generalised}.


\subsubsection{Fixed or random effects}
Several criteria influence whether a hierarchical or grouping variable should be treated as a random or fixed effect in the analysis. Fixed effects are usually used when the analysts are interested in the individual level estimates of a grouping variable \cite{bolker2009generalized} and these are independent, mutually exclusive, and completely observed (for example, control and treatment in experiments, male and female when analyzing differences between sex) (e.g., \cite{hedges1998fixed}; \cite{gunasekara2014fixed}). Random effects, in comparison, are vital modeling choices when the variance between the different levels is of interest \cite{bolker2009generalized} and not the exact estimates of the different levels \cite{dersimonian1986meta}. Random effects can also be employed when not every manifestation of the underlying mechanism can be observed (for example, sampled students from various schools) but the analysts want to adjust for its influence. In this study, the trip IDs are the random factor levels.


\subsubsection{Families}
A key feature of \ac{GAMMs} or GLMMs is the ability to appropriately model a variety of response distributions. They do not make the default assumption that this distribution is Gaussian and therefore require that the researchers specify an appropriate distribution \cite{lo2015transform}. They can handle categorical response variables (binomial), integer response variables (Poisson, negative binomial) right-skewed response variables (gamma, inverse Gaussian, Tweedie), or symmetrical response variables (Gaussian), for example.

\paragraph{Student’s t model}$ $\newline
The t-distribution provides a useful extension of the normal for statistical modeling of data sets involving errors with longer-than-normal tails \cite{lange1989robust}. 
\\\\
The t-distribution is symmetric and bell-shaped, like the normal distribution. However, the t-distribution has heavier tails, meaning that it is more prone to producing values that fall far from its mean.  
\\\\
Estimating the Student’s t model requires estimating another parameter of the distribution, the degrees of freedom (\(\nu\)), the smaller the degrees of freedom the heavier the tails of the conditional distribution of the response. The model is more resistant to more extreme observations because to the thicker tails in this distribution, which have higher probability density until the Student's t with adequate degrees of freedom than the Gaussian.
\\\\
The density of the Gaussian family is given by

\begin{equation}
\begin{aligned}
f(y_i) = \frac{1}{\sqrt{2\pi}\sigma} \textrm{exp} \left(-\frac{1}{2}\left(\frac{y_i-g(\eta_i)}{\sigma}\right)^2\right)
\end{aligned}
\end{equation}


where \(y_i\) and \(\eta_i\) stands for the response and
(non-)linear predictor of observation \(i\), \(f\) for the density function and \(g\) for the inverse link
function, and \(\sigma\) is the residual standard deviation.\\


And the density of the Student’s t family is given by 

\begin{equation}
\begin{aligned}
f(y_i) = \frac{\Gamma((\nu+1)/2)}{\Gamma(\nu/2)}\frac{1}{\sqrt{\nu\pi}\sigma} \left(1+\frac{1}{\nu}\left(\frac{y_i-g(\eta_i)}{\sigma}\right)^2\right)^{-(\nu+1)/2}
\end{aligned}
\end{equation}


where \(y_i\) and \(\eta_i\) stands for the response and
(non-)linear predictor of observation \(i\), \(f\) for the density function and \(g\) for the inverse link
function, \(\nu\) is the number of degrees of freedom and \(\Gamma\) denotes the gamma function. As \(\nu \rightarrow \infty\), the student distribution becomes
the gaussian distribution \cite{burkner2017brms}.


\paragraph{Zero-inflated and hurdle models}$ $\newline
Zero-inflated models and hurdle models, proposed by \cite{mullahy1986specification}, uses a two-stage modeling process. The basic idea is that a binomial model governs the binary outcome of the dependent variable being zero or positive. If the dependent variable takes a positive value, ”hurdle is crossed”, and the conditional distribution of the positives can be modeled by a zero-truncated Poisson or negative binomial model for the count data, for instance.\\


The density of a zero-inflated or hurdle family is given by 
\begin{equation}
\begin{aligned}
f_z(y_i) = g_z(\eta_{zi}) + (1-g_z(\eta_{zi}))f(y_i) \quad \textrm{if} \quad y_i = 0\\
f_z(y_i) = (1-g_z(\eta_{zi}))f(y_i)  \quad \textrm{if} \quad y_i > 0
\end{aligned}
\end{equation}

The zero-inflation part has its own predictor \(\eta_{zi}\) combined with the logit link \(g_z\) \cite{burkner2017brms}.


\subsection{Model estimation}
The standard \ac{ML} is biased for the estimation of variance components. For example, linear mixed-effects model, the conditional response of the response variable \(y\) given \(\beta\), b, \(\theta\), and \(\sigma^2\) is

\begin{equation}
y|b, \beta, \theta, \sigma^2 \sim \mathcal{N}(X\beta+Zb, \sigma^2I_n).
\end{equation}

The likelihood of \(y\) given \(\beta\), \(\theta\) and \(\sigma^2\) is

\begin{equation}
P(y|\beta, \theta, \sigma^2) = \int P(y|b, \beta, \theta, \sigma^2) P(b|\theta, \sigma^2) db.
\end{equation}

The \ac{ML} method treats \(\beta\) as fixed but unknown quantities when the variance components are estimated, but does not take into account the degrees of freedom lost by estimating the fixed effects. This causes \ac{ML} estimates to be biased with smaller variances \cite{pinheiro2006mixed}. \\


The \ac{ML} procedure of \cite{hartley1967maximum} is therefore modified by adapting a transformation from \cite{patterson1971recovery} which partitions the likelihood render normality into two parts, one being free of the fixed effects, and maximization of this provides what is called \ac{REML} estimators of the variance components.\\ 


\ac{REML} estimation includes only the variance components, that is, the parameters that parameterize the random-effects terms in the linear mixed-effects model, \(\beta\) is estimated in a second step. Assuming a uniform improper prior distribution for \(\beta\) and integrating the likelihood \(P(y|\beta, \theta, \sigma^2)\) with respect to \(\beta\) results in the restricted likelihood \(P(y|\theta, \sigma^2)\). That is,

\begin{equation}
P(y|\theta, \sigma^2) = \int P(y|\beta, \theta, \sigma^2) P(\beta) d\beta.
\end{equation}

The algorithm first profiles out \(\hat{\sigma_R}^2\) and maximizes remaining objective function with respect to \(\theta\) to find \(\hat{\theta_R }\). The restricted likelihood is then maximized with respect to \(\sigma^2\) to find \(\hat{\sigma_R}^2\). Then, it estimates \(\beta\) by finding its expected value with respect to the posterior distribution:

\begin{equation}
P(\beta|y, \hat{\theta_R }, \hat{\sigma_R}^2). 
\end{equation}

\ac{REML} accounts for the degrees of freedom lost by estimating the fixed effects and makes a less biased estimation of random effects variances \cite{snijders2011multilevel}. The estimates of \(\theta\) and \(\sigma^2\) are invariant to the value of \(\beta\) and less sensitive to outliers in the data compared to \ac{ML} estimates. However, the comparison of two models is only possible which have identical fixed-effects design matrices and are nested in their random-effects terms \cite{raudenbush2002hierarchical}.


\subsection{Model selection}
Model selection is the process of selecting one final machine learning model from among a collection of candidate machine learning models for a training dataset. The problem with the traditional evaluation metrics such as R-squared (\(R^2\)), \ac{RMSE} is that they are sensitive to the inclusion of additional variables in the model, even if those variables don't have a significant contribution in explaining the outcome \cite{botchkarev2018performance}. Put in other words, including additional variables in the model will always increase the \(R^2\) and reduce the \ac{RMSE}. As a result, a more reliable metric to guide model selection is required. Concerning \(R^2\), there is an adjusted version, called Adjusted R-squared, which adjusts the \(R^2\) for having too many variables in the model. Additionally, there are two other commonly used important metrics - Akaike information criterion (AIC) and Bayesian information criterion (BIC).

\paragraph{\ac{AIC}}$ $\newline
The Akaike information criterion is one of the most common methods of model selection and was introduced by \cite{akaike1998information}. \ac{AIC} weights the ability of the model to predict the observed data against the number of parameters the model requires to reach that level of precision. \ac{AIC} model selection can help find a model that explains the observed variation in their data while avoiding overfitting.
\\\\
\ac{AIC} is defined as:

\begin{equation}
\label{eq:aic}
\textrm{AIC} = -2\mathcal{L}(\hat{\theta}) + 2p
\end{equation}

where \(\mathcal{L}(\hat{\theta})\) is the likelihood of the estimated model, \(p\) is the total number of parameters that are estimated in the model. The smaller values indicate better models. The criteria
balance simplicity (measured by, \(p\), the dimension of the fitted model parameter space) and goodness of fit (measured by maximized likelihood). The most obvious reason why likelihood alone cannot be used to compare models is that models with more free parameters have a higher maximum likelihood.


\paragraph{\ac{BIC}}$ $\newline
The Bayesian information criterion (BIC) (known also as Schwarz Criterion) is another statistical measure for the comparative evaluation among models introduced by \cite{schwarz1978estimating}. When a number of k parameters (regressors or/and intercept) are added to the models, the difference between BIC and AIC becomes apparent, in order to increase the goodness of fit of the model. In such a case, the BIC penalizes more (in comparison to the AIC) such an increase of parameters.\\

BIC is defined as:

\begin{equation}
\label{eq:aic}
\textrm{BIC} = -2\mathcal{L}(\hat{\theta}) + log(n)p
\end{equation}

where \(\mathcal{L}(\hat{\theta})\) is the likelihood of the estimated model, \(p\) is the total number of parameters that are estimated in the model, and \(n\) is the sample size. The smaller values indicate better models. 


\section{Ensemble learning}
Ensemble methods are strategies that construct several models and then combine them to achieve better results than a single model would. This usually results in more accurate solutions than a single model would \cite{NecatiDemir}. There are two well-known effective ensemble methods, bagging and boosting. Bagging is the type of ensemble technique in which a single training algorithm is used on different subsets of the training data where the subset sampling is done with replacement (bootstrap). Once the algorithm is trained on all the subsets, then bagging predicts by aggregating all the predictions made by the algorithm on different subsets. Boosting, on the other hand, is an ensemble strategy for improving any learning algorithm's model predictions. The idea of boosting is to train weak learners sequentially, each trying to correct its predecessor. The weak learners are systematically rectified by their predecessors, converting them into strong learners in the process \cite{JosephRocca}. 


\subsection{Random forest}
\ac{RF}, in general terms, represents a family of methods that consist in building an ensemble (or forest) of decision trees. Random forests (RF henceforth), introduced by \cite{breiman1996bagging}, is a non-parametric statistical learning method from the ensemble decisions trees approaches which is one of the state-of-the-art machine learning methods for prediction and classification. 
\\\\
More specifically, each tree from the random forest is built on a bootstrap sample of the training dataset. Bootstrap sampling also called bagging (from bagged aggregation), exposes the tree construction algorithm to a slightly different subset of the training data for each tree, resulting in a collection of different trees. A small subsample of variables (the mtry parameter in the RF literature) is used at each tree node split, inducing further variation among trees. Together, bagging and variable subsampling reduce overfitting and make RF a more stable classifier than a single decision tree \cite{JasonBrownlee}. The algorithm can be explained by:
\begin{enumerate}
  \item Iteratively construct \(N\) Bootstraps (with replacement) of size \(n\)sampled
from \(Z\), where \(N\) is the number of Bootstrap replicates (trees to grow) and \(Z\) is the
population to draw a Bootstrap sample from.
  \item Grow a random-forest tree \(T_b\)
 at each node randomly select \(m\) variables from \(M\)
to permute through each node to find the best split by using the Gini entropy index
to assess information content and purity. Grow each tree to the full extent with no
pruning (e.g., no complexity parameter). 
  \item Using withheld data (OOB, out-of-bag) to validate each random tree \(T_b\)
 (for classification OOB Error; for regression pseudo \(R^2\) and mean squared error).
 \item Make a prediction for a new observation \(x_i\) for regression, for example: 
 \begin{equation*}
  \hat{f}_{rf}^B(x) = \frac{1}{B} \sum^{B}_{b=1} T_b(x)
  \end{equation*}
\end{enumerate}

\cite{evans2011modeling}. For fitting \ac{RF} on longitudinal data, small modification is proposed by \cite{karpievitch2009introspective} utilizing subject-level bootstrapping, which enables the effective use of all data samples and allows for unequal contribution from the subjects. That is to say, the algorithm grows each tree on a bootstrap sample (a random sample selected with replacement) at the subject level rather than at the replicate level of the training data. It has advantages for the analysis of longitudinal data because the sampling scheme is designed to accommodate data with multiple measurements for a given subject. Also, as the primary goal of the thesis is prediction, and not in performing inference on the model components, the method has shown to be effective in predicting cluster-correlated data. The visualization of the random forest algorithm for clustered data is shown in Figure \ref{fig:RF++}. The hyperparameters for the algorithm are the same as for a normal random forest, and the descriptions of the hyperparameters of the algorithm are shown in Table \ref{tab:hy_rf}.

\begin{figure}[!h]
\centering
\includegraphics[width=13cm, height=8cm]{figures/RF++.png}
\vspace*{5mm}
\caption{Visualization of random forest algorithm applied on clustered data. Figure adapted from \cite{karpievitch2009introspective}.}
 \label{fig:RF++}
\end{figure}


  \begin{table}[htbp]
\caption{Descriptions of hyperparameters of random forest models.}
\vspace*{5mm}
\label{tab:hy_rf}
\centering
\begin{tabular}{>{\itshape}llll}
\toprule % replaced all \hline commands with rules from the booktabs package
\textbf{Hyperparameter}       &  \textbf{Description} \\
\midrule
ntrees    &  Number of decision trees in the forest \\
mtry  &  Number of predictors sampled at each split \\

\bottomrule
\end{tabular}
\end{table}


\subsection{Boosting}
Many researchers have also turned
increasingly to the use of boosting for longitudinal data. For example, using likelihood-based boosting, \cite{tutz2007boosting} described mixed-effects modeling using semi-parametric splines for fixed effects,  while \cite{groll2012regularization} considered generalized additive models subject to P-splines. 
\\\\
A simple approach would be to use the traditional gradient boosting method to form a marginal model as \ac{GEE}. \ac{GEE}, proposed by \cite{liang1986longitudinal}, is a general statistical approach to fit a marginal model for clustered data analysis. Different from the mixed-effect model which is an individual-level approach by adopting random effects to capture the correlation between the observations of the same subject \cite{crowder1995use}, \ac{GEE} is a population-level approach based on a quasi-likelihood function and provides the population-averaged estimates of the parameters \cite{wedderburn1974quasi}. In this method, the correlation between measurements is modeled by assuming a working correlation matrix. The estimations from the GEE are broadly valid estimates that approach the correct value with increasing sample size regardless of the choice of correlation model \cite{overall2004robustness}.
\\\\
More specifically, suppose that longitudinal data consists of \(K\) subjects/clusters. For subject/cluster \(i\) (\(i\) = 1, 2,..., \(K\)), suppose that there are \(n_i\) observations and \(Y_{ij}\) denotes the \(j\)th response (\(j\) = 1,..., \(n_i\)), and let \(X_{ij}\) denotes a \(p \times 1\) vector of covariates. Let \(Y_{i} = (Y_{i1}, Y_{i2},..., Y_{in_i})'\) denote the response vector for the \(i\)th subject with the mean
vector noted by \(\mu_i = (\mu_{i1}, \mu_{i2},..., \mu_{in_i})'\) where \(\mu_{ij}\) is the
corresponding \(j\)th mean. The responses are assumed to be independent across subjects/clusters but correlated within each subject/cluster. The marginal model specifies that a relationship between \(\mu_{ij}\) and the covariates \(X_{ij}\) is written as follows:
\begin{equation}
g(\mu_{ij}) = {X'_{ij}} \boldsymbol{\beta}
\end{equation}

where \(g\) is a known link function and \(\boldsymbol{\beta}\) is an unknown \(p \times 1\) vector of regression coefficients with the true value as \(\boldsymbol{\beta}_0\). The conditional variance of \(Y_{ij}\) given \(X_{ij}\) is specified
as Var(\(Y_{ij}|X_{ij}\)) = \(v(\mu_{ij})\phi\), where \(v\) is a known variance function of \(\mu_{ij}\) and \(\phi\) is a scale parameter which may need to
be estimated. Mostly, \(v\) and \(\phi\) depend on the distributions of outcomes.  Also, the variance-covariance matrix for \(Y_i\) is noted by \(V_i = \phi A_i^{1/2}R_i(\boldsymbol{\alpha})A_i^{1/2}\), where \(A_i\) = Diag\{\(v(\mu_{i1}),...,v(\mu_{in_i}))\)\} and the so-called “working” correlation structure \(R_i(\boldsymbol{a})\) describes the pattern of measures within subject, which is of size \(n_i \times n_i\) and depends on a vector of association parameters denoted by \(\boldsymbol{\alpha}\). The iterative algorithm is applied for estimating \(\boldsymbol{\alpha}\) using the Pearson residuals \(e_{ij} = (y_{ij} - \mu_{ij}) / \sqrt{v(\mu_{ij})}\) calculated from the current value of \(\boldsymbol{\beta}\). The scale parameter \(\phi\) can be estimated by
\begin{equation}
\hat{\phi} = \frac{1}{N-p}\sum^{K}_{i=1} \sum^{n_i}_{j=1} e^2_{ij}
\end{equation}
where \(N = \sum^{K}_{i=1}n_i\) is the total number of observations and \(p\) is covariates dimensionality. The estimate of \(\boldsymbol{\beta}\) is obtained by
solving the following estimating equation:
\begin{equation}
U(\boldsymbol{\beta}) = \sum^{K}_{i=1} D'_i V_i^{-1} (Y_i - \mu_i) = 0
\end{equation}
where \(D_i = \partial \mu_i / \partial \boldsymbol{\beta}'\) \cite{wang2014generalized}.
\\\\
The model fitting process of boosting algorithm used in the thesis is similar to using GEE with a diagonal working-covariance matrix. If \(F_k\) is the model at the \(k\)th boosting iteration, a regression tree is fit to the residuals \(r_{ij} = y_{ij} - F_k(x_{ij})\) for \(i = 1,...,n\) and \(j = 1,...,n_i\) (n subjects and \(i\)th subject observed at \(n_i\) time points). If \(T_{k+1}\) denotes this regression tree, then the model is updated by \(F_{k+1}=F_{k}+T_{k+1}\), and the procedure is repeated. Determining the number of boosting iterations is done by using cross-validation with a leave-out-subject approach. The descriptions of the hyperparameters for boosting models are shown in Table \ref{tab:hy_tb}.

 \begin{table}[htbp]
\caption{Descriptions of hyperparameters of boosting models.}
\vspace*{5mm}
\label{tab:hy_tb}
\centering
\begin{tabular}{>{\itshape}llll}
\toprule % replaced all \hline commands with rules from the booktabs package
\textbf{Hyperparameter}       &  \textbf{Description} \\
\midrule
ntrees    &  Number of decision trees in ensemble \\
nsplit  &  Number of splits in each regression tree \\
lambda  &  Shrinkage parameter applied to each tree \\
\bottomrule
\end{tabular}
\end{table}



\subsection{Variable importance}
A variety of variable importance measures for ensemble learning models have been proposed (e.g., \cite{sandri2008bias}; \cite{archer2008empirical}). The most direct way of assessing the importance of a variable is to refit the model with the variable excluded.
The relative change in the prediction error due to the variable deletion can then
be computed and used to measure its importance. However, the drawback of the delete variable importance measure is computational, since to compute it for all variables, the model needs to be refit for each one. An alternative to refitting
the model with the \(k\)th predictor removed, is to marginalize the model. This marginalized model is

\begin{equation}
\label{eq:aic}
m_k(x) = \int m(x)dP_k(x)
\end{equation}

where \(m_k(x)\) is the model estimate obtained after removing
the \(k\)th predictor from the data, \(m(x)\) is the model estimate using all the predictors, and \(P_k\) is the empirical distribution of the predictor \(k\). The importance of this variable can then be measured as the (relative) change in prediction error due to its marginalization \cite{htree}.




\section{Validation}
\subsection{Leave-one-out Cross-validation (LOOCV)}
Cross-validation is a resampling method that uses different portions of the data to test and train a model on different iterations. The cross-validation has a single hyperparameter “k” that controls the number of subsets that a dataset is split into \cite{refaeilzadeh2009cross}. Once split, each subset is given the opportunity to be used as a test set while all other subsets together are used as a training dataset. \ac{LOOCV}, is an extreme version of k-fold cross-validation that has the maximum computational cost. It requires one model to be created and evaluated for each example in the training dataset \cite{wong2015performance}.\\

Cross-validation is crucial where the amount of data available is limited. Compare with the traditional train and test split: use the first 75 percent (three blocks) of the data as the training data set and the last 25 percent (one block) as the testing data set, which users don't know what is the best way to determine the training and testing dataset, and different train-test splits of the data can lead to completely
distinct results. Cross-validation lets data scientists use all of the data without sacrificing any subset and reveals the consistency of the data and the algorithm \cite{AmalJoby}. The last but not the least is that it helps avoid overfitting and underfitting of the models to the data.


\subsection{Absolute percentage error}
\ac{APE} is utilized for the cumulative values of the energy consumption at time point \(T\) of a trip (i.e., the end time of a trip), and is defined as:
\begin{equation}
\textrm{APE}_T = \bigg|\frac{y_T - f_T}{y_T}\bigg|
\end{equation}

where \(y_T\) is the real value and \(f_T\) is the forecast value at time \(T\).

==> tool.tex <==
\chapter{Tools}\label{tool}
The chapter describes the tool chain that has been set up to conduct the whole data analysis procedure, including the links to download the software.

\section{MATLAB}
The battery electric vehicle model is implemented in MATLAB, and the simulation process is done by using MATLAB Engine API for Python. The MATLAB Engine API for Python provides a package named matlab for Python to call MATLAB as a computational engine. The source code in Python can be found in Appendix \ref{appendix:MATLAB}.

\section{R}
The machine learning corrective models are written purely in R. The packages in R provide plenty of functionalities for data visualization and data modeling.
\\\\   
R is freely distributed online, and one can download it from the R homepage, which is:
\url{https://cran.r-project.org/}. For the application to interact with R, one can download Rstudio from: \url{https://www.rstudio.com/}. A screenshot of Rstudio running on a Windows is shown in Figure \ref{fig:rstudio} in Appendix \ref{appendix:R}. Some of the important packages and functions used in this thesis can also be found in Appendix \ref{appendix:R}.



